Deadlock Freedom for Asynchronous and Cyclic Process Networks

This paper considers the challenging problem of establishing deadlock freedom for message-passing processes using behavioral type systems. In particular, we consider the case of processes that implement session types by communicating asynchronously in cyclic process networks. We present APCP, a typed process framework for deadlock freedom which supports asynchronous communication, delegation, recursion, and a general form of process composition that enables specifying cyclic process networks. We discuss the main decisions involved in the design of APCP and illustrate its expressiveness and flexibility using several examples.

==> eptcsdata.tex <==
\providecommand{\firstpage}{38}
\providecommand{\publicationstatus}{J. Lange, A. Mavridou, L. Safina, A. Scalas (Eds.):\\
14th Interaction and Concurrency Experience (ICE 2021).\\
EPTCS 347, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.347.3}{10.4204/EPTCS.347.3}}

